Passive Self-Interference Suppression for Full-Duplex Infrastructure Nodes

Recent research results have demonstrated the feasibility of full-duplex wireless communication for short-range links. Although the focus of the previous works has been active cancellation of the self-interference signal, a majority of the overall self-interference suppression is often due to passive suppression, i.e., isolation of the transmit and receive antennas. We present a measurement-based study of the capabilities and limitations of three key mechanisms for passive self-interference suppression: directional isolation, absorptive shielding, and cross-polarization. The study demonstrates that more than 70 dB of passive suppression can be achieved in certain environments, but also establishes two results on the limitations of passive suppression: (1) environmental reflections limit the amount of passive suppression that can be achieved, and (2) passive suppression, in general, increases the frequency selectivity of the residual self-interference signal. These results suggest two design implications: (1) deployments of full-duplex infrastructure nodes should minimize near-antenna reflectors, and (2) active cancellation in concatenation with passive suppression should employ higher-order filters or per-subcarrier cancellation.

==> characterization_old_v2.tex <==
%\section{Passive Suppression Characterization Results}
\section{Experiment Results}
\label{sec:characterization}

Let us first consider the measurements of the achieved passive suppression in Configuration~\dirBigA\  (Figure~\ref{fig:config_90_50}), in which $90\degree$ beamwidth transmit antennas are used with transmit and receive antennas pointed $90\degree$ apart. Table~\ref{tab:EnvironmentComparison} shows the average passive suppression $\bar\alpha^{(\mathsf{mech})}_{\rm P}$ in the ISM band for four different combinations of passive suppression mechanisms, $\mathsf{mech} \in \{\mathsf{\emptyset, D, DA, DC, DCA}\}$. All but the first row of Table~\ref{tab:EnvironmentComparison} are measurements from Configuration~\dirBigA which uses $90~\degree$ beamwidth antennas with $90~\degree$ separation. 
In order to evaluate the benefit of the directional isolation inherent to Configuration~\dirBigA, Table~\ref{tab:EnvironmentComparison} also lists the measured suppression for Configuration~\omniBig, which uses omnidirectional antennas and not other suppression mechanisms ($\mathsf{mech = \emptyset}$).
%In order get an idea for how much passive suppression is coming from the directional isolation in Configuration~\dirBigA\ the first row lists the passive suppression measurement for the Configuration~\omniBig with antennas spaced the same distance, as in Configuation~\omniBig. 


\renewcommand{\arraystretch}{1.5}
\begin{table}[htdp]
\caption{Average Suppression Measurements, Directional Configurations}
\begin{center}
%\begin{tabular}{c c}
\subfigure[\normalsize{\underline{Anechoic Chamber}}]{
	\begin{tabular}{|l||>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|}
\hline
	Applied Mechanism ($\mathsf{mech}$) & Config~\dirBigA & Config~\dirBigB & Config~\dirSmall \tabularnewline \hline \hline
	Directional $(\sf D)$ & 45.3~dB  &  39.7~dB & 46.2~dB \tabularnewline \hline
	${\sf D}$ + Absorber $(\sf DA)$ & 55.4~dB &  50.9~dB & 55.9~dB \tabularnewline \hline
	${\sf D}$ + Cross-polarization $(\sf DC)$ & 63.9~dB  &  58.3~dB & 56.9~dB\tabularnewline \hline
	${\sf D}$ + Cross-pol + Absorber $(\sf DCA)$ & 73.8~dB & 72.5~dB & 72.4~dB \tabularnewline \hline
	${\sf D}$ + ${\sf A}$ + Reflector $(\sf DAR)$ & 61.7~dB  & 57.7~dB & -- \tabularnewline \hline
	${\sf D}$ + ${\sf C}$ + ${\sf A}$ + Reflector $(\sf DCAR)$ & 71.7~dB & 73.1~dB & -- \tabularnewline \hline
	% The metal shield data for config DirBigB and DirSmall were the same, which means that one is repeat of the other. I'm pretty sure that DirSmall is repeat of DirBig. 
	\end{tabular}
	\label{tab:DirChamber}
	}
\subfigure[\normalsize{\underline{Reflective Room}}]{
	\begin{tabular}{|>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|}
\hline
	 Config~\dirBigA & Config~\dirBigB & Config~\dirSmall \tabularnewline \hline \hline
	 37.7~dB & 36.0~dB & 37.1~dB \tabularnewline \hline
	 39.4~dB & 38.1~dB & 37.4~dB \tabularnewline \hline
	 45.1~dB & 44.9~dB & 44.4~dB \tabularnewline \hline
	 45.9~dB & 44.9~dB & 45.7~dB \tabularnewline \hline
	 40.2~dB & 38.1~dB & 40.0~dB \tabularnewline \hline
	 45.8~dB & 45.0~dB & 46.5~dB \tabularnewline \hline
	\end{tabular}
	\label{tab:DirRoom}
	}
\end{center}
%\end{tabular}
\end{table} 


%\begin{figure}[htbp]
%\begin{center}
%\subfigure[Anechoic Chamber]{
%	\input{suppressionPlotDirChamber.tex}
%}\subfigure[Reflective Room]{
%	\input{suppressionPlotDirRoom.tex}
%}
%\caption{Passive suppression measurements}
%\label{fig:suppression}
%\end{center}
%\end{figure}

\begin{figure}[htbp]
\begin{center}
\subfigure[Anechoic Chamber]{
	\input{suppressionPlotDirChamber_2.tex}
}\subfigure[Reflective Room]{
	\input{suppressionPlotDirRoom_2.tex}
}
\caption{Passive suppression measurements for directional configurations}
\label{fig:suppression}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\subfigure[Anechoic Chamber]{
	\input{suppressionPlotOmniChamber_2.tex}
}\subfigure[Reflective Room]{
	\input{suppressionPlotOmniRoom_2.tex}
}
\caption{Passive suppression measurements for omnidirectional configurations}
\label{fig:suppression}
\end{center}
\end{figure}
	
\renewcommand{\arraystretch}{1.5}
\begin{table}[htdp]
\caption{Average Suppression Measurements, Omnidirectional Congifurations}
\begin{center}
%\begin{tabular}{c c}
\subfigure[\normalsize{\underline{Anechoic Chamber}}]{
	\begin{tabular}{|l||>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|}
	\hline
	Applied Mechanism ($\mathsf{mech}$)& Config~\omniBig & Config~\omniSmall \tabularnewline \hline \hline
	None $(\sf \emptyset)$ & 27.9~dB & 24.5~dB\tabularnewline \hline
	Absorber $(\sf A)$ & 48.0~dB & 48.2~dB \tabularnewline \hline
	Absorber + Reflector $(\sf AR)$ & 62.9~dB & 65.8~dB \tabularnewline \hline
	% The metal shield data for config DirBigB and DirSmall were the same, which means that one is repeat of the other. I'm pretty sure that DirSmall is repeat of DirBig. 
	\end{tabular}
	\label{tab:OmniChamber}
	}
\subfigure[\normalsize{\underline{Reflective Room}}]{
	\begin{tabular}{|>{\centering}p{1.2cm}|>{\centering}p{1.2cm}|}
	\hline
	Config~\omniBig & Config~\omniSmall \tabularnewline \hline \hline
 	27.6~dB & 25.1~dB \tabularnewline \hline
	40.1~dB & 41.1~dB \tabularnewline \hline
	41.6~dB & 42.4~dB \tabularnewline \hline
	\end{tabular}
	\label{tab:OmniRoom}
	}
\end{center}
%\end{tabular}
\end{table} 





Let us first look at the first column of measurements in Table~\ref{tab:EnvironmentComparison} which were performed in the anechoic chamber.  We see in the second row of Table~\ref{tab:EnvironmentComparison} that when Configuration~\dirBigA\ is used without any absorptive shielding or cross-polarization, the average passive self-interference suppression is 45~dB. Comparing to the average passive suppression in the omnidirectional configuration of Configuration~\dirBigB\ in the first row, we see that the directional isolation inherent to Configuration~\dirBigA\ is providing around 17~dB of passive suppression in addition to the 28~dB of path loss between antennas. 
%Path loss between antennas at this distance is around 30~dB, so the directional isolation inherent to the configuration is providing around 15~dB of suppression.
Adding absorptive shielding between antennas in addition to the directional isolation gives an extra 10~dB of suppression for 55~dB total suppression. Similarly, cross-polarization in addition to the directional isolation gives an extra 18~dB of suppression for a total suppression of 66~dB. When all the  mechanisms are applied in tandem, directional isolation absorptive shielding, and cross-polarization together yield 74~dB total suppression, which leads us to the following result. 

\begin{result}
\label{result:noAnalog}
In a low-reflection environment, combining directional isolation, absorptive shielding, and cross-polarization achieves sufficient passive suppression to remove the need for analog-domain self-interference cancellation at WiFi ranges. \note{(Not sure if I want this here, but we will see.)}
\end{result}

\begin{proof}[Reason for Result~\ref{result:noAnalog}]
\note{(If actually going to use this, must make it much the reason more convincing)} Previous full-duplex designs have employed analog self-interference cancellation because the self-interference is assumed to be several orders of magnitude more powerful that the received signal-of-interest. Digital self-interference is considered insufficient because the ADC must expand its dynamic range to accommodate the high-powered self-interference signal, resulting in heavy quantization noise on the low-powered signal-of-interest. %leaving only a few bits of precision for representing the lower-powered signal-of-interest.  
Experimental characterizations have shown \note{[cite]} that the path loss encountered in typical WiFi deployments ranges from 60~dB to 80~dB. If the self-interference is passively suppressed by 60-75~dB as shown in Table~\ref{tab:EnvironmentComparison}, then the signal-of-interest and the self-interference will have similar power levels, making it possible to simple quantize the received signal and cancel the self-interference digitally. 
More precisely, assuming path loss between 60 and 80~dB and passive self-interference suppression of 74~dB, the power differential between the signal-of-interest and the self-interference in a typical WiFi deployment will be between -6~dB and 14~dB. In the worst case of the signal-of-interest, being down 6~dB from the self-interference only 1 bit of precision is lost. This one bit of precision is far below the noise floor in typical deployments, and this quantization error is not a problem. 
\end{proof}



%\renewcommand{\arraystretch}{1.5}
%\begin{table}[htdp]
%\caption{Passive Suppression Measurements for Configuration~\dirBigA} 
%\begin{center}
%\ifCLASSOPTIONtwocolumn
%	\begin{tabular}{|m{2.5cm}|m{1.5cm}|m{1.5cm}|}
%\else
%	\begin{tabular}{|l|>{\centering}p{3.0cm}|>{\centering}p{3.0cm}|}
%\fi
%
%\hline
%Applied Mechanism(s) & Average Suppression (Anechoic Chamber) & Average Suppression (Reflective Room)\tabularnewline \hline \hline
%Omnidirectional (Config~\omniBig) & $27.9$ dB		& $27.8$ dB	\tabularnewline \hline
%$90\degree$ Directional (Config~\dirBigA)	& $45.2$ dB	    & $38.5$ dB	\tabularnewline \hline
%Directional + Absorber						& $55.2$ dB 	& $41.2$ dB	\tabularnewline \hline
%%Dir.+Abs.+Shield	& $61.7$ dB 	& $--$ dB		& $--$ dB	\tabularnewline \hline
%Directional + Cross-polarization			& $64.3$ dB		& $46.1$ dB	\tabularnewline \hline
%Directional + Cross-polarization + Absorber & $74.5$ dB 		& $46.7$ dB \tabularnewline \hline
%%Dir.+Abs.+Shield+ Cross-pol 	& $72.5$ dB 	& $46.1$ dB	& $--$ dB	\tabularnewline \hline
%\end{tabular}
%\end{center}
%\label{tab:EnvironmentComparison}
%\end{table}








%\subsection{Anechoic Chamber Measurements}
%\begin{result}
% This is the first results
%\end{result}
%\begin{reason}
% This is the reason for the result
%\end{reason}
%\begin{principle}
%Here's the resulting design principle. 
%\end{principle}



==> conlusion.tex <==
\section{Conclusion}
\label{sec:discussion}
%\EvanNote{Conclusion is coming soon.}
We have seen that a careful utilization of the passive self-interference suppression mechanisms of directional isolation, absorptive shielding, and cross-polarization can significantly improve the performance of full-duplex links, but some fundamental limitations are encountered. The amount of passive suppression is limited by reflected paths which are difficult to predict and suppress passively. Moreover, because passive suppression eliminates the once-dominant direct self-interference path, but leaves the reflected paths, the residual self-interference channel can be much more frequency selective than the original self-interference channel. We have shown that a design that takes these capabilities and limitations into account can achieve a full-duplex link that outperforms a comparable half-duplex link even a ranges exceed 100~m. 
%\EvanNote{Should we even do a conclusion?}\AshuNote{This looks fine.}
